ChatGPT versus Traditional Question Answering for Knowledge Graphs: Current Status and Future Directions Towards Knowledge Graph Chatbots

Conversational AI and Question-Answering systems (QASs) for knowledge graphs (KGs) are both emerging research areas: they empower users with natural language interfaces for extracting information easily and effectively. Conversational AI simulates conversations with humans; however, it is limited by the data captured in the training datasets. In contrast, QASs retrieve the most recent information from a KG by understanding and translating the natural language question into a formal query supported by the database engine. In this paper, we present a comprehensive study of the characteristics of the existing alternatives towards combining both worlds into novel KG chatbots. Our framework compares two representative conversational models, ChatGPT and Galactica, against KGQAN, the current state-of-the-art QAS. We conduct a thorough evaluation using four real KGs across various application domains to identify the current limitations of each category of systems. Based on our findings, we propose open research opportunities to empower QASs with chatbot capabilities for KGs. All benchmarks and all raw results are available1 for further analysis.

==> Sections/benchmarks.tex <==
\subsection{Benchmarks}
\label{sec:Benchmarks}

Our evaluation used different benchmarks, two on general-fact KGs, namely  DBpedia~\cite{DBpedia}, YAGO\footnote{\url{https://yago-knowledge.org/downloads/yago-4}}~\cite{yago}, and another two benchmarks on KGs related to academia, namely DBLP\footnote{\url{https://dblp.org/rdf/release/dblp-2022-06-01.nt.gz}} and the Microsoft Academic Graph (\emph{MAG})\footnote{\url{https://zenodo.org/record/4617285\#.YrNszNLMJhH}}. The general-fact KGs have facts about entities representing places and persons. DBLP and MAG contain facts about scientific publications, citations, authors and institutions. Each benchmark includes a set of English questions against one of these four KGs. Each question is annotated with the equivalent SPARQL query and the answers to the question. These answers are retrieved by executing the given SPARQL query. The benchmarks consist of different categories of questions, such as boolean questions whose answer is $True$ or $False$, listing questions where the answer should contain an exhaustive list of KG entities answering the question, and WH-questions that ask about people, places, languages, etc.

We used {\qald}~\cite{qald9}, the most challenging and widely used benchmark to evaluate QASs.  {\qald} uses the DBpedia KG, and consists of $150$ questions for testing. The questions of {\qald} are human-generated. The other benchmarks, namely YAGO, DBLP, and MAG, are recently introduced by \cite{KGQan}. Each of these benchmarks contains $100$ questions for testing. These questions are also human-generated, following the same type of questions in  {\qald}. The questions against YAGO are similar to the ones of  {\qald}, i.e.,  questions about people and places. Both DBLP and MAG benchmarks have questions related to citations and authors. 




% To evaluate and compare {\chatgpt} with {\kgqan} in the KGQA task, we used four benchmarks developed for four different graphs:  {\qald}, and YAGO on general knowledge graphs, DBLP, and MAG on academic graphs.
% Each data instance in the benchmarks consists of: the question text, the equivalent SPARQL query, and the answers to the question, these answers are retrieved by executing the given SPARQL query. Each benchmark is developed on a specific version of the knowledge graph because KGs are frequently updated by adding new entities and relations, so the same SPARQL query may have a different set of answers if executed on two versions of the same KG. The benchmarks consist of different categories of questions, such as boolean questions whose answer is $True$ or $False$, listing questions where the answer should contain an exhaustive list of KG entities answering the question, and WH-questions that ask about people, places, languages, etc.

% {\qald} \cite{qald9} is a well-known benchmark used for evaluating KGQA systems. It is developed on DBpedia graph version $10$-$2016$. It consists of $408$ questions for training and $150$ for testing. The questions of {\qald} are human-generated, so the length of the questions is not long, the average length of questions is $7.5$ words.  
% The other benchmarks are recently introduced in \cite{KGQan}, they are created following the same process as {\qald}, and each of them consists of $100$ questions used for testing since {\kgqan} does not need to be trained on the benchmarks.
% YAGO benchmark is developed on the YAGO4 version of the YAGO graph. It is another general knowledge benchmark that contains questions about people and places.
% DBLP is developed on top of the $06$-$2022$ version of the DBLP graph, It contains questions asking about citations, scientific publications, and authors. 
% MAG is developed on the $05$-$2020$ version of the Microsoft Academic Graph, which is another example of a large academic graph. Similar to DBLP, its questions ask about citations and authors.



==> Sections/discussion.tex <==
\section{Discussion}
% \begin{itemize}
%     \item If we had access to the pre-trained chatGTP model, and we were allowed to train it further with our training set, could we potentially improve its QA capabilities?
%     \item KG-QA systems query directly the KG to retrieve answers. chatGTP, on the other hand, uses the information that was available during training. What are the possible advantages and disadvantages?
%     \item Is chatGTP more ``universal'' than KGQan?
% \end{itemize}

From the previous results, it is clear that {\chatgt} fails with dealing with detailed information from a specific domain such as the academic domain as in most of the questions that it cannot provide answers to, it mentions that it was not trained on these information. If we have access to the pre-trained {\chatgpt} model, and we re-train it on academic information, it is more likely to answer more questions in the benchmarks. {\chatgpt} can achieve better performance if it was fine-tuned to produce all results of listing questions. Currently when there is a question that has hundreds of answers, {\chatgpt} mentions that there are a lot of answers for this questions but it only gives a small subset of 20 answers maximum and this affected its recall.

KGQA systems directly query the KG to retrieve the answers, while {\chatgpt} uses the information it was trained on to answer the question. One advantage of the {\chatgpt} technique is the ability to answer questions from different sources, while in case of KGQA if the information is not in the target KG, it won't be able to answer the question. Another advantage of {\chatgt} is its ability to have a conversation with the user if the questions needs clarification or update. One disadvantage is incorporating new knowledge in {\chatgt} in case we are dealing with data sources that are updated frequently, this will require fine-tuning the model which will exhaust a lot of time and resources. On the other hand {\kgqan} can work with multiple new KGs directly without the need of doing any training or processing.

{\kgqan} is a universal framework that can work with different knowledge graphs and different domains, On the other hand {\chatgpt} is not universal with respect to different domains as in its current state it can work perfectly with only general knowledge information.





==> Tables/dblp_runs.tex <==
\begin{table}[t]
    \caption{Performance of {\chatgpt} across three runs on {DBLP}, where $C$ means that the question was answered correctly, $W$ means the question was not answered correctly and $NA$ means that {\chatgpt} failed to return any useful answer}
  \label{tab:dblpruns}
  \centering
  
\begin{tabular}{lccc}
\hline
\textbf{Run 1} & \textbf{Run 2} & \textbf{Run 3} & \textbf{Count} \\
\hline
C & C & C & 3 \\
C & NA & C & 1 \\
C & NA & NA & 1 \\
C & W & W & 1 \\
W & C & NA & 1\\
\hline
NA & NA & NA & 87 \\
W & NA & NA & 1 \\
W & NA & W & 1 \\
W & W & W & 4 \\
\hline
\end{tabular}
\end{table}


==> Tables/yago_runs.tex <==
\begin{table}[t]
    \caption{Performance of {\chatgpt} across three runs on {YAGO}, where $C$ means that the question was answered correctly, $W$ means the question was not answered correctly and $NA$ means that {\chatgpt} failed to return any useful answer}
  \label{tab:dblpruns}
  \centering
  
\begin{tabular}{lccc}
\hline
\textbf{Run 1} & \textbf{Run 2} & \textbf{Run 3} & \textbf{Count} \\
\hline
C & C & C & 49 \\
C & C & W & 2 \\
C & NA & C & 2 \\
C & W & W & 1 \\
NA & NA & C & 1 \\
W & C & C & 3 \\
W & C & W & 1 \\
\hline
NA & NA & NA & 22 \\
NA & W & NA & 3 \\
W & NA & NA & 1 \\
W & W & NA & 1 \\
W & W & W & 14 \\
\hline
\end{tabular}
\end{table}

